CONSTRUCT: A Program Synthesis Approach for Reconstructing Control Algorithms from Embedded System Binaries in Cyber-Physical Systems

We introduce a novel approach to automatically synthesize a mathematical representation of the control algorithms implemented in industrial cyber-physical systems (CPS), given the embedded system binary. The output model can be used by subject matter experts to assess the system's compliance with the expected behavior and for a variety of forensic applications. Our approach first performs static analysis on decompiled binary files of the controller to create a sketch of the mathematical representation. Then, we perform an evolutionary-based search to find the correct semantic for the created representation, i.e., the control law. We demonstrate the effectiveness of the introduced approach in practice via three case studies conducted on two real-life industrial CPS.

==> BK/Background.tex <==
\section{Background \& Problem Definition}
\label{sec:Background}



Cyber-physical system designers use tools such as Simulink~\citeme{}, Matlab~\citeme{}, and OpenModelica~\citeme{} to design models and simulate their behavior in various situations. Then, the designed model and its corresponding simulation can be exported by these tools as a standardized portable package called \textit{Functional Mockup Unit (FMU)} that is transportable from one simulator to the other. An FMU contains binary files (e.g., compiled C files) that implement the functionality of the cyber-physical system, alongside some text-based description files which provide information about the modeled cyber-physical system (e.g., information on inputs, outputs, and other internal variables used in the system). In this paper, we consider the FMU of a cyber-physical system as the input to our approach. There are three main reasons behind this decision listed below:
\begin{itemize}
    \item FMU is a well-respected and standardized container for exchanging and co-simulating dynamical models.
    \item There are a vast number of modeling tools that support FMU exportation including Matlab, Simulink, Dymola, OpenModelica, SimulationX, and more.
    \item An FMU container can include both source code as well as binaries targeting different platforms.
\end{itemize}

\begin{figure}[ht]
  \centering
  \includegraphics[width=.49\textwidth]{figures/Problem_Definition.pdf}
  \caption{Synthesizing mathematical representations of a given cynber-physical system in form of an FMU.}
  \label{fig:Problem_Definition}
\end{figure}

Figure~\ref{fig:Problem_Definition} shows the expected input and output of the proposed approach in this paper. We define the problem of this paper as: \textbf{\textit{Given an FMU of a cyber-physical system, we aim to develop an approach that generates mathematical representations of the given system. The synthesized mathematical representation shall follow the syntax and semantic of Modelica language~\citeme{}, which is a multi-domain modeling language for component-oriented modeling of complex systems and is easily interpretable by subject matter experts (SME) that are not necessarily familiar with programming languages, but are experts in understanding the behavior of cyber-physical systems.}} The synthesized mathematical representations shall be intuitive such that even a person with a non-advanced mathematical knowledge can understand the behavior of the cyber-physical system in generating the output(s) from the given input(s).



\subsection{Motivating Example}
\label{sec:Motivation}
\ali{To be added.}

==> BK/CONSTRUCT.tex <==
\section{CONSTRUCT}
\label{sec:Construct}
To address the mentioned challenges in understanding the behavior of cyber-physical systems, in this paper, we introduce our novel \textbf{Code-based MOdel SyNthesiS PlaTform foR re-ConstrUcting Control AlgoriThms} \textsc{\textbf{(CONSTRUCT)}} which automatically constructs mathematical representations of controller parts of cyber-physical systems. Figure~\ref{fig:CONSTRUCT} shows an overview of this approach. 
In summary, \textsc{CONSTRUCT} takes-in an FMU file which contains binaries and some descriptions about the cyber-physical model. 
The main idea is to create the structure of the mathematical model from the decompiled codes through AST translation, and then find the correct mappings between symbolic names and the actual variable names by leveraging an evolutionary search technique, Genetic Algorithm.
From the description files inside the FMU, \textsc{CONSTRUCT} identifies the variable names that should be used in the final mathematical model and some attributes of those variables. Then, it decompiles the binary files inside the FMU and localizes the mathematical primitives that are commonly used in controller parts of Cyber-physical systems. Next, it creates the AST of the decompiled sources and translates sub-ASTs that correspond to mathematical primitives to mathematical-formed ASTs. Note that through the decompilation process, the original variable names will be replaced with non-real symbolic names. We use Genetic Algorithm as an evolutionary search-based approach to find a correct mapping between the generated symbolic names of variables in the created mathematical representation and the original variable names retrieved from the description file inside the FMU. The output of \textsc{CONSTRUCT} is a mathematical representation that complies with syntax and semantic of Modelica modeling language. The Modelica language is vastly used for mathematical modeling purposes and provides opportunity for simulating mathematical models. 
We provide details on each step of \textsc{CONSTRUCT} as follows.

\begin{figure}[ht]
  \centering
  \includegraphics[width=.25\textwidth]{figures/CONSTRUCT_new.pdf}
  \caption{An overview of the \textsc{CONSTRUCT} approach.}
  \label{fig:CONSTRUCT}
\end{figure}

\subsection{Step 1: Binary Decompilation}
\ali{To be added by Shantanu/Peter.}

\subsection{Step 2: Mathematical Primitive Isolation \ali{Localization?}}
\ali{To be added by Shantanu/Peter.}

\subsection{Step 3: Transforming Code-level ASTs to Model-level ASTs}
\ali{To be added by Shantanu/Peter.}

\subsection{Step 4: Modelica Model Synthesis}
Since the original FMU is given as an input to \textsc{CONSTRUCT}, we can provide inputs to the FMU and receive its corresponding outputs. Although we have not a clear idea on the behavior of the FMU at this point, we can still rely on the binaries inside the FMU as an important source of information that we use while synthesizing the mathematical model. We basically use this FMU as an oracle to make sure that the synthesized mathematical model correctly represents the behavior of the cyber-physical system.
From the previous steps, we were able to create the structure of the mathematical representation, including equations and symbolic variable names. Moreover, from the description file of the FMU, we were able to collect the required information (e.g., name, type, etc.) on the variables that should be used in the equations. 

In this step, we aim to find a correct mapping between variable names and symbolic variables such that by providing the same input to the given FMU and the synthesized mathematical model, their output also be the same. Note that some of the variables in equations can be independent variables (e.g., they are not derivations of other variables), some might be derivations of the independent variables or other type of calculated variables, and the rest can be parameters i.e., constant values that their value remains unchanged regardless of the value of the input or output or other variables.

\subsubsection{Correct by Testing}
%\subsubsubsection{Problem Formulation}

In order to solve the mapping problem through genetic algorithm (GA), we need to first translate the original mapping problem as a GA problem, find a proper solution, and then, translate back the solution to a solution for the mapping problem. In a GA problem, one should represent possible solutions in the form of a \textit{chromosome}, which basically is a sequence of so-called \textit{genes}. Figure~\ref{fig:GA_Problem_Formulation} shows how we formulate our mapping problem as a GA problem.   

\begin{figure*}[h]
  \centering
  \includegraphics[width=.9\textwidth]{figures/GA_Problem_Formulation.pdf}
  \caption{The genetic algorithm problem formulation. }
  \label{fig:GA_Problem_Formulation}
\end{figure*}

\begin{itemize}
    \item \textbf{Solution representation:} 
 In our approach, we consider the length of a chromosome as the same as the number of symbolic variables that are present in the mathematical model, and each gene represents a variable number from the list of the variables that we extracted from the description file of the FMU (figure~\ref{fig:GA_Problem_Formulation}(a)). For instance, if the third gene in the chromosome equals number 5, it means that we assign the fifth variable in the variable list to the third symbol in the symbol list. Following this solution representation, even in the simple equation demonstrated in \secref{sec:Motivation} that has 3 equations, 12 symbols, and 13 variables, the number of possible solutions to explore is $12!$, around $480M$. Please note that upon finding a solution (i.e., a mapping between symbols and variables), one has to generate the equation, create an FMU based on the equation, and simulate the created FMU by providing inputs to receive its corresponding outputs. This process is a mandatory part of the approach to make sure about the correctness of the synthesized mathematical representation. Due to the mentioned over head in this process, it would not be feasible to explore all the possible solutions to find the best one. In fact, we use the power of GA to avoid such exploration.     
    
    \item \textbf{First population generation:} We randomly generate the first population, meaning that random numbers of variables will be assigned to random symbols (figure~\ref{fig:GA_Problem_Formulation}(b)). However, we make sure that no two genes in a chromosome have the same variable number. This ensures that each symbol will be assigned a unique variable in the synthesized mathematical representation. Moreover, at the end of this process, all the symbols will have one variable assigned to them. 

    \item \textbf{Mutation operation:}
    In order to mutate a chromosome, we randomly select two genes in the chromosome, and swap their value. Figure~\ref{fig:GA_Problem_Formulation}(c) demonstrates this process. 
    
    \item \textbf{Cross-over operation:}
    Given two chromosomes, we randomly select a crossing point and concatenate the first part of first parent to the second part of second parent, and also the first part of second parent to the second part of the first parent to create new children from the given two parents (figure~\ref{fig:GA_Problem_Formulation}(d)). \ali{Any guarantee on not appearance of a variable more than once in the children?}
    
    \item \textbf{Fitness:} In our approach, the fitness is a little bit different from the common sense of the fitness score which is the higher the fitness is, the better is the solution. In our case, the fitness is basically the distance between the output of the generated model with the output of the given FMU. Therefore, the lower the fitness is, we consider the found solution as more valuable. 

\end{itemize}

Following the explained approach, we expect to achieve better solutions (i.e., solutions with lower errors) through next generations. In other words, starting from the early generations, we might find symbol-variable mappings such that the output of their created FMUs have a considerable distance to the output of the given FMU. However, moving forward, we would like to see that the found mappings result in mathematical representations with lower distance between their output and the output of the original FMU. Finally, we would like to see that at some point, the output of the synthesized mathematical representation completely matches the output of the given FMU. However, as will explain further, this is not always the case.

\subsubsection{Correct by Construction}

In order to calculate the fitness of the generated chromosomes, we use the \textit{OpenModelica} to simulate the synthesized mathematical model and compare the output of the simulation against the simulation output of the reference FMU. To be simulatable, the synthesized mathematical model must follow certain syntax and semantic rules of \textit{Modelica} language . Otherwise, OpenModelica throws an exception and does not return an output. Nevertheless, during the individual (i.e., chromosome) generation by the baseline \textit{Correct by Testing} method, we observed that a considerable number of created mathematical representations do not comply with the expected syntax or semantic of Modelica language. In particular, we identified the following issues that can result in creation of non-simulatable mathematical representations. To mitigate these challenge, we followed the \textit{Correct by Construction} paradigm in which we make sure that all the operations in our GA approach generate simulatable solutions. 

\begin{itemize}
    \item \textit{Different types of variables:} We observed that it is quite possible that the symbolic, as well as actual variables in the equations might be from different types (e.g. Real, Boolean, or String). In such cases, we can not arbitrarily assign a variable to a symbol without considering the type compliance constraint. For example, whenever we find a symbolic statements such as the following, we infer that the type of the variable that will be assigned to $Symbol_2$ should be of type \textit{Boolean}:
    $Symbol_1 = if(Symbol_2) Symbol_3 else Symbol_4;$
    \item \textit{At least one independent variable per equation:} To be able to simulate the generated mathematical model, the OpenModelica requires all the equations to at least include one independent variable. Otherwise, the equation would be considered as too trivial and the simulation will not be carried out. 
    \item \textit{Equal number of the independent variables and the equations:} Another constraint that OpenModelica puts on the generated mathematical models is that the total number of independent variables used in the model should be equal to the number of the equations. Otherwise, the equation system would be considered as under- (in case that the number of variables is less than the number of equations) or over-estimation (in case that the number of variables is greater than the number of equations) and the simulation will not happen.
    \item \textit{Usage of I/O variables in the equations:} Another important constraint is that all the input and output variables should be used in the equations.  
\end{itemize}

By generating chromosomes that syntactically and semantically comply with Modelica language, we basically changed the paradigm of our synthesizer from \textbf{\textit{Correct-by-Testing}} to \textbf{\textit{Correct-by-Construct}}. In other words, instead of synthesizing models that we are not sure about their soundness, we changed our synthesis approach such that it only generates mathematical models that are \textbf{sound}, i.e., the model is simulatable by the simulator. 

==> BK/CaseStudyBK.tex <==
\section{Case Study}
\label{sec:PreliminaryResult}
In order to showcase the performance of the introduced approach, in this section, we present case studies conducted on three different controllers used in two real-world cyber-physical systems, a \textit{Turtlebot Waffle Pi}~\citeme{} which is a inherently stable wheeled robot, and a \textit{PX4 Quadcopter}~\citeme{} which is statically unstable robot. In each case, we first provide information on the controller, and then, we share the results of the conducted experiment. Figure~\ref{fig:correct_by_construct_result} summarizes the result of this study. In our experiments, the population size was considered as 400 and the maximum number of generations was 10. 
%
\begin{figure}[ht]
%   \vspace{-2pt}
  \centering
  \includegraphics[width=.49\textwidth]{Case_Study.pdf}
  \caption{The result of synthesizing mathematical models based on the Correct-by-Testing (base-line) and our Correct-by-Construct approach.}
  \label{fig:correct_by_construct_result}
%   \vspace{-10pt}
\end{figure}
%
\subsection{Case \#1: PI Controller}
\ali{Needs more information and characteristics of the system. }
The first case shown in figure~\ref{fig:correct_by_construct_result} corresponds to a model with 8 equations, 18 variables, and 23 symbols. The orange curve represents the performance of the correct-by-testing approach, and the blue curve  shows the result of correct-by-construction approach. Clearly, even in this case that all the variables and symbols are from the same type (i.e., Real), the correct-by-construct approach is able to find better mathematical representations.

\subsection{Case \#2: PID Controller}
However, by adding to the complexity of the models, the true power of correct-by-construction would be visible. \ali{Needs more information and characteristics of the system.}
In this case, there were 6 equations, 37 variables, and 20 symbols, and more than one type in the equations. As shown in figure~\ref{fig:correct_by_construct_result}.b, the correct-by-testing approach was not able to generate even one single chromosome that can be simulated using the simulator. However, not only the correct-by-construct approach can generate such models, it also finds solutions with relatively good scores.

\subsection{Case \#3: LimPID Controller}
\ali{Needs more information and characteristics of the system. }
Finally, Case \#3 shows a more complex system compared to Cases \#1 and \#2. Even in this case, the correct-by-construct approach can generate simulatable solutions while the correct-by-testing approach cannot. 

==> BK/Conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}

==> BK/ExperimentalStudy.tex <==
\section{Case Study}
\label{sec:ExperimentalStudy}
In order to showcase the performance of the introduced approach, in this section, we conduct three case studies on real-world cyber-physical systems. In each case, we first provide information on the system, and then, we share the results of the conducted experiment. Figure~\ref{fig:correct_by_construct_result} summarizes the result of this study.   

\subsection{Case \#1: DC Motor}
\ali{Needs more information and characteristics of the system. }
The first case shown in figure~\ref{fig:correct_by_construct_result} is for a model with 8 equations, 18 variables, and 23 symbols. The orange curve represents the performance of the Correct-by-Testing approach, and the blue curve is shows the result of performing the mentioned changes and shifting the paradigm to Correct-by-Construct. Clearly, even in this case that all the variables and symbols are from the same type (Real), the Correct-by-Construct approach is able to find better mathematical representations by end of the run of the approach.

\subsection{Case \#2: PID}
However, by adding to the complexity of the models, the true power of the performed changes would be visible. \ali{Needs more information and characteristics of the system.}
In this case, there were 6 equations, 37 variables, and 20 symbols, and more than one type in the equations in the Case \#2 (PID model). In this case, the Correct-by-Testing approach was not able to generate even one single chromosome that can be simulated using the simulator. However, not only the Correct-by-Construct approach is able to generate such models, but also it finds solutions with relatively good scores.


\subsection{Case \#3: PID Lim}
\ali{Needs more information and characteristics of the system. }
Finally, Case \#3 shows a more complex system compared to Case \#1 and \#2. However, the Correct-by-Construct approach can generate simulatable solutions for this case while the Correct-by-Testing approach cannot. 


\begin{figure*}[ht]
  \centering
  \includegraphics[width=.8\textwidth]{correct_by_construct_result.pdf}
  \caption{The result of changing the synthesis paradigm from Correct-by-Testing to Correct-by-Construct.}
  \label{fig:correct_by_construct_result}
\end{figure*}







==> BK/Introduction.tex <==
\section{Introduction}
\label{sec:Introduction}
Cyber-physical systems are composed of different components, including physical as well as computational parts. One important component of such systems is a software that glues everything together and aims to control the interactions and performs needed processing.
These systems are used in very important mission- and safety-critical domains such as military, medical, transportation, and agriculture.
Therefore, it is crucial to make sure that these software have been correctly implemented and they behave as they are expected. In particular, it is important to investigate this issue before using the system in practice.
Undoubtedly, one way to find a knowledge on what the software does is to read the code and find an insight into the implemented functionality. However, even an expert programmer cannot easily sit in a session and read the code of a software and find a clear idea on the software's functionality. More importantly, most of these systems are delivered in the format of binary codes. Hence, one needs to de-compile the binaries first, and generate its source code to be reviewed. However, through the de-compilation process, the generated source code will be obfuscated, meaning that variable names, method names, and even in some cases class names are changed to meaningless and strange names which makes it dramatically hard to follow the code.

Cyber-physical system designers use tools such as Simulink~\citeme{}, Matlab~\citeme{}, and OpenModelica~\citeme{} to design models and simulate their behavior in various situations. Then, the designed model and its corresponding simulation can be exported by these tools as a standardized portable package called \textit{Functional Mockup Unit (FMU)} that is transportable from one simulator to the other. An FMU contains binary files (e.g., compiled C files) that implement the functionality of the cyber-physical system, alongside some text-based description files which provide information about the modeled cyber-physical system (e.g., information on inputs, outputs, and other internal variables used in the system). 
In this paper, we consider the FMU of a cyber-physical system as the input to our approach. There are three main reasons behind this decision listed below:
\begin{itemize}
    \item FMU is a well-respected and standardized container for exchanging and co-simulating dynamical models.
    \item There are a vast number of modeling tools that support FMU exportation including Matlab, Simulink, Dymola, OpenModelica, SimulationX, and more.
    \item An FMU container can include both source code as well as binaries targeting different platforms.
\end{itemize}

We define the problem of this paper as: \textbf{\textit{Given an FMU of a cyber-physical system, we aim to develop an approach that generates mathematical representations of the given system. The synthesized mathematical representation shall follow the syntax and semantic of Modelica language~\citeme{}, which is a multi-domain modeling language for component-oriented modeling of complex systems and is easily interpretable by subject matter experts (SME) that are not necessarily familiar with programming languages, but are experts in understanding the behavior of cyber-physical systems.}} The synthesized mathematical representations shall be intuitive such that even a person with a non-advanced mathematical knowledge can understand the behavior of the cyber-physical system in generating the output(s) from the given input(s).

To address these challenges, in this paper, we report our efforts on automatically synthesizing a high-level mathematical representation of the behavior of the software component of cyber-physical systems, especially the control part. The ultimate goal in this project is to support non-programmer Subject Domain Experts (SMEs) to be able to easily and effortlessly understand the behavior of the given cyber-physical system to investigate whether the software works as it is expected or not. This can facilitate identification of possible drifts from the intended specification of the system and avoid unwanted behaviors (e.g., a cyber-physical system is malicious or weaponized). 




==> BK/Limitations.tex <==
\section{Limitations and Future Work}
\label{sec:Limitations}

==> BK/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> BK/RelatedWork.tex <==
\section{Related Work}
\label{sec:RelatedWork}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip

